VisEval: A Benchmark for Data Visualization in the Era of Large Language Models

Translating natural language to visualization (NL2VIS) has shown great promise for visual data analysis, but it remains a challenging task that requires multiple low-level implementations, such as natural language processing and visualization design. Recent advancements in pre-trained large language models (LLMs) are opening new avenues for generating visualizations from natural language. However, the lack of a comprehensive and reliable benchmark hinders our understanding of LLMs' capabilities in visualization generation. In this paper, we address this gap by proposing a new NL2VIS benchmark called VisEval. Firstly, we introduce a high-quality and large-scale dataset. This dataset includes 2,524 representative queries covering 146 databases, paired with accurately labeled ground truths. Secondly, we advocate for a comprehensive automated evaluation methodology covering multiple dimensions, including validity, legality, and readability. By systematically scanning for potential issues with a number of heterogeneous checkers, VisEval provides reliable and trustworthy evaluation outcomes. We run VisEval on a series of state-of-the-art LLMs. Our evaluation reveals prevalent challenges and delivers essential insights for future advancements.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/benchmark_old.tex <==
\section{Benchmark Goal}
% Benchmark Requirements 
In this section, we point out the scope of our benchmark and summarize benchmark requirements accordingly.

\subsection{Evaluation Scope}
In the era of large language models, a prevalent workflow of NL2VIS is assembling a query along with data tables, then soliciting LLMs to generate code based on visualization libraries.
This code snippet serves as an intermediary step, leading to the creation of the final visualization image. 
Therefore, to conduct a comprehensive evaluation of the quality of generated visualizations, it is imperative to assess each checkpoint, encompassing both the code and the resulting chart image.
We frame the evaluation scope within established Python visualization, such as Matplotlib~\cite{hunter2007matplotlib} and Seaborn~\cite{waskom2021seaborn}. 
These visualization libraries are widely used and offer the flexibility to create diverse visualizations.

To better understand the primary dimensions needed for automated evaluations, we conducted a pre-study with two experts who have six years of experience in visualization. 
Five hundred queries were randomly sampled from nvBench~\cite{luo2021synthesizing} and used to generate visualizations using four different LLMs (e.g., GPT-4, GPT-3.5, Gemini-Pro, CodeLlama-7B). Following this, two authors and two experts independently reviewed the codes and chart images generated by each of the four models. 
Subsequently, a roundtable meeting was convened to discuss the findings of all evaluators.
Finally, we classified the common issues into three dimensions based on previous literature related to visualization linting~\cite{chen2021vizlinter,mcnutt2018linting,hopkins2020visualint} and code generation benchmark~\cite{zhang2024benchmarking, lai2023ds}.

\noindent\textbf{I1.~Invalid codes lead to rendering failure.} The generated code may be invalid for rendering visualizations, such as crashing during execution (e.g., due to incorrect API usage or syntax errors) or lacking the necessary code to render the visualizations (e.g., printing transformed data instead of plotting them).

\noindent\textbf{I2.~Illegal charts do not meet requirements.} When the visualization is rendered, it may still be illegal due to conflicts with queries, such as wrong data transformations (e.g., incorrect attributes, performing improper aggregations), wrong visualization transformations (e.g., inappropriate visual mappings, missing legends), or not sorting as required.

\noindent\textbf{I3.~Low readability charts hinder comprehension.} Even if a chart seems to fulfill the requirements of visualization, it can still encounter challenges that impede comprehension from various perspectives. These challenges may include layout issues (such as text overflow or overlap), axis problems (like using unconventional floating numbers to represent years), difficulties with colors (such as low contrast making it difficult to distinguish elements), and typos.


Upon discovering that the current generation still exhibits numerous basic errors, we decided to focus our efforts on evaluating the capabilities of LLMs in generating visualizations, particularly in instances where queries explicitly define attributes, aggregations, chart types, and order.
This is crucial due to the inherent flexibility of natural language queries, which often leads to non-unique ideal visualizations and poses challenges for reliable evaluation. 
We firmly believe that our evaluation process constitutes a fundamental and indispensable component of NL2VIS assessment.
The assessment of vague queries can be effectively decomposed into multiple steps to ensure reliable results. 
For instance, when a query lacks specificity regarding visualization type, we propose a division into separate evaluations for visualization recommendation and generation. Similarly, in cases where data attributes remain unspecified, we advocate for distinct evaluations focused on auto-insight and generation.

% Besides, we note that the flexibility inherent in natural language queries often results in non-unique ideal visualizations, thus presenting challenges for evaluation. 
% % Such queries can encompass explicit, partially explicit, or implicit references to data attributes, visualizations, and order requirements.
% To address this complexity, we advocate for breaking down the evaluation of NL2VIS into multiple steps. 
% For instance, when a query lacks specificity regarding visualization type, we propose a division into separate evaluations for visualization recommendation and generation. Similarly, in cases where data attributes remain unspecified, we advocate for distinct evaluations focused on auto-insight and generation.
% The primary objective of this paper is to assess the capabilities of LLMs in generating visualizations, particularly in instances where queries explicitly specify attributes, aggregations, chart types, and order. This evaluation constitutes the fundamental and indispensable component of NL2VIS assessment.

% \subsection{Preliminaries}
% % problem definition
% % current issues
% The nvBench~\cite{luo2021synthesizing} benchmark, known for its extensive and broad-domain coverage, has been widely employed in the evaluation of various NL2VIS methods~\cite{song2022rgvisnet, li2024prompt4vis, cheng2023gpt,maddigan2023chat2vis1,li2024visualization}.
% Recently, two works~\cite{maddigan2023chat2vis1,li2024visualization} utilize nvBench to automatically assess the accuracy of code generated by LLMs for matplotlib~\cite{hunter2007matplotlib} and Vega-Lite~\cite{satyanarayan2016vega}, respectively.
% They employed a similar evaluation method: LLMs generated code using queries from nvBench. The generated code was then converted into SVG images, facilitating the extraction of underlying x and y-axis data. This extracted data was subsequently compared to the ground truth, resulting in match accuracy.


% \input{tables/nvbench_issues}
% However, we identify several issues with nvBench. 
% As highlighted in the preceding works~\cite{maddigan2023chat2vis1,li2024visualization}, inaccuracies in the ground truth data of nvBench can lead to an unfair evaluation of accurate codes. And certain queries rely on empty data tables, causing failures in code execution.
% Furthermore, NL queries in nvBench also suffer from issues such as ambiguity, irrationality, and redundancy. 
% For example, there is a query with the ID \textit{21}, ``Show the number of male and female assistant professors''. The ground truth chart type for this query is a pie chart. However, due to the unclear specification of the chart type in the query, LLMs might generate a bar chart, which is also a valid choice, labeling it as a mismatch would be unjust. 
% More detailed examples of each issues type are provided in Table ~\ref{tab:benchmark-shortcomings}.


% Meanwhile, the previous automatic evaluation method that simply compares whether x and y-axis data match with ground truth also lacks correctness, fairness, and comprehensiveness.

% \noindent\textbf{I1.~Correctness.} Chat2vis~\cite{maddigan2023chat2vis1} highlights the potential for unfair results in direct comparisons, particularly when, after sorting, multiple x values share the same y value, resulting in multiple valid sorting outcomes.
% Variations in time formats may also result in erroneous comparisons, such as using ``mon'' as an abbreviation for ``Monday'' or representing it directly with the number ``1''. 
% Moreover, not comparing all data comprehensively may result in false positives. For instance, missing or incorrectly drawn legends, or using the same color for different categories, as shown in (\cref{fig:evalution_issues}(a)) with ``Creative Labs'' and ``Hewlett-Packard'' sharing the same color 
% \begin{tikzpicture}
%   \fill[legend] (0,0) circle (0.1cm);
% \end{tikzpicture}
% , can make the chart invalid.

% \noindent\textbf{I2.~Fairness.}
% Most queries do not explicitly indicate which attributes are mapped to the x and y axes, which aligns with the characteristic of how people express queries~\cite{srinivasan2021collecting}.
% However, this can lead to unfair results, as a single query may correspond to multiple valid visual mapping choices. 
% For instance, when drawing a bar chart as a horizontal bar, the x and y axes are swapped. 
% Specifically, as illustrated in (\cref{fig:evalution_issues}(b)), the data field ``Rank'' is mapped to color channel, and ``Sex'' is mapped to the x-axis in the generated chart. In contrast, the ground truth indicates that ``Sex'' is mapped to color channel, and ``Rank'' is mapped to the x-axis.

% \noindent\textbf{I3.~Comprehensiveness.} 
% % During our practical evaluation, we identified issues in visualizations generated by LLMs, which extend beyond the assessment of information correctness. 
% Beyond information correctness, the overall quality of visualizations is influenced by various perspectives.
% During our practical evaluation, we found that readability issues demand careful attention, exemplified by challenges such as text overflowing, inappropriate choice of ticks, and lack of a title, as shown in~\cref{fig:casestudy}(c).
% Previous works have primarily focused on the correctness of visualizations generated by LLMs, overlooking these readability-related issues.

% In response to the identified issues, we augment the benchmark, and introduce a reliable evaluation framework designed to ensure fair evaluation and provide insights into the readability of the generated visualizations.
% In this paper, we prioritize readability in our evaluation, temporarily excluding other aspects like aesthetics and memorability. 
% Due to the limited stylistic diversity in the current generated visualizations, aesthetics and memorability are considered less of a primary concern.
% In the future, we incorporate those aspects into our framework for a more comprehensive assessment.


\subsection{Benchmark Requirements}
% Benchmark Specification / core features
\label{sec:design_goals}
% highlight three core features
To reliably evaluate visualizations based on the three dimensions mentioned above, we highlight three requirements as follows.

\noindent\textbf{R1. Provide a high-quality and large-scale dataset.} The benchmark dataset should be large in scale and board in domain, encompassing diverse domains of databases and chart types, while also avoiding the inclusion of low-value duplicates to prevent bias. Additionally, the dataset should demonstrate high quality, with accurately annotated ground truth, non-ambiguous queries and reasonable visualizations.

\noindent\textbf{R2. Support multi-criteria evaluation metrics.} Evaluating generated visualization requires comprehensive consideration from various perspectives. Some prior approaches~\cite{maddigan2023chat2vis1,li2024visualization} focused solely on metrics that compare data along the x and y axes to ground truth, often overlooking critical issues such as missing legends or the use of identical colors for distinct categories. For instance, as illustrated in \cref{fig:evalution_issues}(a), the categories ``Creative Labs'' and ``Hewlett-Packard'' are depicted in the same color \begin{tikzpicture}
  \fill[legend] (0,0) circle (0.1cm);
\end{tikzpicture}, leading to the misrepresentation of data in the chart.
Therefore, it is imperative that we systematically evaluate the visualizations for validity (\textbf{I1}), legality (\textbf{I2}), and readability (\textbf{I3}).


\noindent\textbf{R3. Automate reliable evaluation.} The outcomes are truly valuable only when the evaluation is reliable, but it is challenging to automate the evaluation of generated visualizations reliably. Despite specifying the chart type in the query, the visualizations generated are not unique, as they can have different visual mappings. For instance, in \cref{fig:evalution_issues}(b), it is also appropriate to map the sex attribute to the color channel, and the rank attribute to the x-axis. Assessing readability reliably is even more challenging, as it involves considering various aspects such as layout, scale, and color, which are difficult to achieve through predefined rules.

% \noindent\textbf{G1. High-quality queries with trustworthy ground truth.} As our focus is on explicit visualization generation tasks, rather than visualization recommendation or automatic insight, we aim for queries in the benchmark to explicitly describe data transformations and chart types. Additionally, we seek descriptions of reasonable visualizations, trustworthy ground truth, and avoidance of excessive duplication to prevent resource waste and bias.
% To achieve this, we enhanced nvBench by correcting erroneous ground truth, modifying or removing ambiguous or unreasonable queries, removing duplicates, and adding meta-information to describe explicitly mentioned details in the queries.

% \noindent\textbf{G2. Reliable and thorough automated evaluation.} 
% Correctness and fairness are fundamental to a benchmark, and misclassifying either correct results as incorrect or incorrect results as correct is deemed unacceptable. Additionally, since the quality of visualizations is influenced by factors beyond correctness, a thorough evaluation becomes essential to gain profound insights into a model's capabilities. Consequently, we designed a framework that incorporates both information correctness and readability for a comprehensive and reliable assessment.

% \noindent\textbf{G3. Flexible usage and easy integration.} 
% We employ GPT-4-Vision for evaluating the readability of visualizations, as detailed in Section~\ref{sec:readability_checker}. However, access to resources for LLMs is restricted, and we strive to prevent this limitation from hindering the evaluation process. Meanwhile, as previously discussed, evaluating visualizations encompasses various aspects. Therefore, our designed evaluation framework consists of multiple visualization checkers that are configurable and integratable. This flexibility enables users to tailor checks based on their resources, determining the aspects to inspect. Additionally, users can customize checks for additional aspects.



\begin{figure}[t]
    \centering    \includegraphics[width=\linewidth]{figs/examples.pdf}
    \vspace{-3mm}
    \caption{Examples of two queries and generated visualizations. (a) The categories ``Creative Labs'' and ``Hewlett-Packard'' are depicted in the same color. (b) The legal visualizations are not unique, as the mapping of the sex attribute to the color channel and the rank attribute to the x-axis is also considered appropriate. }
    \label{fig:evalution_issues}
    \vspace{-5mm}
\end{figure}






==> tables/comparision_format.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{c|c|c|cc|ccc|ccc}
\toprule
\multirow{2}*{Table formats} & \multirow{2}*{Benchmark} & \multirow{2}*{Pass Rate}& \multicolumn{2}{c|}{Validity} & \multicolumn{3}{c|}{Legality} & \multicolumn{3}{c}{Readability}  \\
& \begin{tabular}{@{}c@{}}\end{tabular} & \begin{tabular}{@{}c@{}}\end{tabular} &  \begin{tabular}{@{}c@{}}Code \\ Error\end{tabular} & \begin{tabular}{@{}c@{}}Display \\ Error\end{tabular} & \begin{tabular}{@{}c@{}}Type \\ Mismatch\end{tabular}  & \begin{tabular}{@{}c@{}}Data \\ Mismatch\end{tabular} & \begin{tabular}{@{}c@{}}Order \\ Mismatch\end{tabular} & \begin{tabular}{@{}c@{}}Layout \\ Issues\end{tabular}  & \begin{tabular}{@{}c@{}}Scale \\ Issues\end{tabular} & \begin{tabular}{@{}c@{}}Score \\\end{tabular} \\ 
\midrule
Chat2vis & Single Table & {\cellcolor[HTML]{8aa485}} \color[HTML]{000000} 70.35  & {\cellcolor[HTML]{fcf6f6}} \color[HTML]{000000} 4.31  & {\cellcolor[HTML]{ffffff}} \color[HTML]{000000} 0.00  & {\cellcolor[HTML]{fdf9f9}} \color[HTML]{000000} 2.85  & {\cellcolor[HTML]{f6e2e2}} \color[HTML]{000000} 14.19  & {\cellcolor[HTML]{f8e9e9}} \color[HTML]{000000} 10.92  & {\cellcolor[HTML]{eec8c8}} \color[HTML]{000000} 26.80 \\
LIDA & Single Table & {\cellcolor[HTML]{8ca688}} \color[HTML]{000000} 68.99  & {\cellcolor[HTML]{fcf7f7}} \color[HTML]{000000} 3.96  & {\cellcolor[HTML]{ffffff}} \color[HTML]{000000} 0.00  & {\cellcolor[HTML]{fefcfc}} \color[HTML]{000000} 1.83  & {\cellcolor[HTML]{f5dfdf}} \color[HTML]{000000} 15.56  & {\cellcolor[HTML]{f8e8e8}} \color[HTML]{000000} 11.31  & {\cellcolor[HTML]{f0cece}} \color[HTML]{000000} 24.06   \\
Coml4vis & Single Table & {\cellcolor[HTML]{8fa88a}} \color[HTML]{000000} 67.46  & {\cellcolor[HTML]{fcf5f5}} \color[HTML]{000000} 4.81  & {\cellcolor[HTML]{ffffff}} \color[HTML]{000000} 0.00  & {\cellcolor[HTML]{fdf9f9}} \color[HTML]{000000} 3.26  & {\cellcolor[HTML]{f4dcdc}} \color[HTML]{000000} 16.97  & {\cellcolor[HTML]{f8eaea}} \color[HTML]{000000} 10.37  & {\cellcolor[HTML]{f1d1d1}} \color[HTML]{000000} 22.40  \\
\hline
Chat2vis & All & {\cellcolor[HTML]{94ac90}} \color[HTML]{000000} 64.37  & {\cellcolor[HTML]{faf0f0}} \color[HTML]{000000} 7.72  & {\cellcolor[HTML]{ffffff}} \color[HTML]{000000} 0.01  & {\cellcolor[HTML]{fefbfb}} \color[HTML]{000000} 2.27  & {\cellcolor[HTML]{f4dcdc}} \color[HTML]{000000} 17.04  & {\cellcolor[HTML]{f8e9e9}} \color[HTML]{000000} 10.73  & {\cellcolor[HTML]{efcdcd}} \color[HTML]{000000} 24.58 \\
LIDA & All & {\cellcolor[HTML]{96ae92}} \color[HTML]{000000} 63.03  & {\cellcolor[HTML]{faf0f0}} \color[HTML]{000000} 7.65  & {\cellcolor[HTML]{ffffff}} \color[HTML]{000000} 0.00  & {\cellcolor[HTML]{fefcfc}} \color[HTML]{000000} 1.60  & {\cellcolor[HTML]{f3d9d9}} \color[HTML]{000000} 18.41  & {\cellcolor[HTML]{f8e9e9}} \color[HTML]{000000} 10.79  & {\cellcolor[HTML]{f1d1d1}} \color[HTML]{000000} 22.64   \\
Coml4vis & All & {\cellcolor[HTML]{98af94}} \color[HTML]{000000} 62.07  & {\cellcolor[HTML]{faeeee}} \color[HTML]{000000} 8.35  & {\cellcolor[HTML]{ffffff}} \color[HTML]{000000} 0.00  & {\cellcolor[HTML]{fdfafa}} \color[HTML]{000000} 2.55  & {\cellcolor[HTML]{f3d9d9}} \color[HTML]{000000} 18.49  & {\cellcolor[HTML]{f8e9e9}} \color[HTML]{000000} 10.86  & {\cellcolor[HTML]{f2d5d5}} \color[HTML]{000000} 20.6  \\
\end{tabular}%
}
\caption{Comparison of different table formats. }
\label{tab:compare-formats}
\end{table*}



==> tables/comparision_llms_readability.tex <==

\begin{table}[t]
\centering
\small
\caption{Comparison of error rates (\%) including layout issue and scale (and ticks) issues, and readability score across different models. ``\# VIS'' columns show the number of passed visualization. 
% The "Layout Issue" and "Scale Issue" columns respectively indicate the rate of occurrences of layout issues and scale and ticks issues. 
% The "Readability Score" on the rightmost represents the overall readability score.
}
\vspace{-2mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|c|cc|c}
\toprule
{Model} & {Library} & \# VIS & Layout Issue $\downarrow$ & Scale Issue $\downarrow$ & {Readability Score $\uparrow$}\\

\midrule
CodeLlama-7B & \multirow{4}*{Matplotlib} & 434  & {\cellcolor[HTML]{f3d8d8}} \color[HTML]{000000} 20.59  & {\cellcolor[HTML]{e6b0b0}} \color[HTML]{000000} 28.34  & {\cellcolor[HTML]{64ae6d}} \color[HTML]{000000} 3.87\\
Gemini-Pro &  & 673  & {\cellcolor[HTML]{fefdfd}} \color[HTML]{000000} 13.56  & {\cellcolor[HTML]{e4a9a9}} \color[HTML]{000000} 29.69  & {\cellcolor[HTML]{429d4d}} \color[HTML]{000000} 3.95\\
GPT-3.5 &  & 797  & {\cellcolor[HTML]{db8b8b}} \color[HTML]{000000} 35.51  & {\cellcolor[HTML]{da8989}} \color[HTML]{000000} 35.88  & {\cellcolor[HTML]{f7fbf7}} \color[HTML]{000000} 3.52\\
GPT-4 &  & 919  & {\cellcolor[HTML]{f9ecec}} \color[HTML]{000000} 16.70  & {\cellcolor[HTML]{da8787}} \color[HTML]{000000} 36.33  & {\cellcolor[HTML]{82be89}} \color[HTML]{000000} 3.80\\
\hline
CodeLlama-7B & \multirow{4}*{Seaborn} & 299  & {\cellcolor[HTML]{eabcbc}} \color[HTML]{000000} 26.11  & {\cellcolor[HTML]{e19f9f}} \color[HTML]{000000} 31.61  & {\cellcolor[HTML]{c5e1c8}} \color[HTML]{000000} 3.64\\
Gemini-Pro &  & 698  & {\cellcolor[HTML]{fdf8f8}} \color[HTML]{000000} 14.56  & {\cellcolor[HTML]{e2a1a1}} \color[HTML]{000000} 31.24  & {\cellcolor[HTML]{60ac69}} \color[HTML]{000000} 3.88\\
GPT-3.5 &  & 796  & {\cellcolor[HTML]{db8c8c}} \color[HTML]{000000} 35.25  & {\cellcolor[HTML]{df9797}} \color[HTML]{000000} 33.21  & {\cellcolor[HTML]{d5e9d8}} \color[HTML]{000000} 3.60\\
GPT-4 &  & 743  & {\cellcolor[HTML]{ebbebe}} \color[HTML]{000000} 25.74  & {\cellcolor[HTML]{e8b4b4}} \color[HTML]{000000} 27.57  & {\cellcolor[HTML]{64ae6d}} \color[HTML]{000000} 3.87 \\
\bottomrule
\end{tabular}%
}

\label{tab:compare_models_readability}
\end{table}
